Planning Landscape Analysis for Self-Adaptive Systems

To assure performance on the fly, planning is arguably one of the most important steps for self-adaptive systems (SASs), especially when they are highly configurable with a daunting number of adaptation options. However, there has been little understanding of the planning landscape or ways by which it can be analyzed. This inevitably creates barriers to the design of better and tailored planners for SASs. In this paper, we showcase how the planning landscapes of SASs can be quantified and reasoned, particularly with respect to the different environments. By studying four diverse real-world SASs and 14 environments, we found that (1) the SAS planning landscapes often provide strong guidance to the planner, but their ruggedness and multi-modality can be the major obstacle; (2) the extents of guidance and number of global/local optima are sensitive to the changing environment, but not the ruggedness of the surface; (3) the local optima are often closer to the global optimum than other random points; and (4) there are considerable (and useful) overlaps on the global/local optima between landscapes under different environments. We then discuss the potential implications to the future work of planner designs for SASs.

==> study.tex <==




\section{Study Methodology}
\label{sec:study}




%Since one of our purposes is to demonstrate how fitness landscape analysis can be useful for understanding the planning landscape of SASs, 

In this work, we seek to answer the following research questions:

\begin{itemize}

\item \textbf{RQ1:} Do the planning landscapes offer useful guidance to a SAS planner under different environments?

\item \textbf{RQ2:} What are the general structural properties of planning landscapes for SASs under different environments?

\item \textbf{RQ3:} Do the local optima closer to global optimum than other non-optimal points in the SAS planning landscape?

\item \textbf{RQ4:} Is it possible to share some information of the planning landscapes for SAS across different environments?

\end{itemize}


%the first research question we aim to answer is:
%
%\begin{rqbox}
%  \noindent
%  \textit{\textbf{RQ1:} Do the planning landscapes offer useful guidance to a SAS planner under different environments?}
%\end{rqbox}
%
%\textbf{RQ1} can provide insights on the selection/design of the SAS planners and their planning algorithms. To further explore this point, an extended question is:
%
%
%
%\begin{rqbox}
%  \noindent
%  \textit{\textbf{RQ2:} What are the general structural properties of planning landscapes for SASs under different environments?}
%\end{rqbox}
%
%\textbf{RQ2} informs us the (relative) likelihood that a planner/planning algorithm may get stuck at local optima, which may help to reason about the necessity of some dedicated ``escaping'' design, such as random perturbation with a larger radius, more rapid random restart, or accepting more inferior adaptation plans in the search.
%
%Although local optima may trap the planner, they can also be useful as, given the sparsity of SAS planning for configurable systems~\cite{ChenMMO21,nair2018finding}, finding some local optima may help reveal the ``path'' towards the global optimum. Hence, in \textbf{RQ3}, we ask:
%
%\begin{rqbox}
%  \noindent
%   \textit{\textbf{RQ3:} Do the local optima closer to global optimum than other non-optimal points in the SAS planning landscape?}
%  %\textit{\textbf{RQ3:} Does the overall distance from local optima to global optimum smaller than that from the other points (except global optima) in SAS planning landscape?}
%\end{rqbox}
%
%Finally, we are interested in understanding what is the relationship between the local and global optimum in the landscapes under different environments for SASs, for which the question is:
%
%%Finally, we are interested in, through analyzing the planning landscapes, whether it is possible to reuse the information of local optima and global optimum in SAS planning across changing environments, for which the question is:
%
%%of local and global optimum
%\begin{rqbox}
%  \noindent
%  \textit{\textbf{RQ4:} Is it possible to share some information of the planning landscapes for SAS across different environments?}
%\end{rqbox}


To that end, as shown in Table~\ref{tb:sys}, we consider three or four environments that can change arbitrarily at runtime for four real-world SAS and use the same setting as previous work. In particular, we exploit the readily available dataset of those systems~\cite{nair2018finding,DBLP:conf/mascots/JamshidiC16,DBLP:conf/sigsoft/JamshidiVKS18,DBLP:journals/corr/abs-2106-02716} which contain the samples for the entire planning landscape of each environment.

% All experiments are repeated 50 runs.

For interpreting the FDC and Correlation Lengths (\textbf{RQ1} and \textbf{RQ2}), we adopt Fisher's transformation~\cite{fisher1915frequency} to find the z-score, which is then interpreted using Zou's confidence interval~\cite{zou2007toward} under a significance level of $0.05$. We leverage the non-paired Wilcoxon rank-sum test at $\alpha=0.05$ for comparing the distance in \textbf{RQ3}. 


%
%\subsection{Subject SASs}
%
%We study four real-world SASs that are widely used in prior work, as presented in Table~\ref{tb:sys}.
%
%
%\textsc{Apache Storm:} a distributed stream processing computation framework that executes a series of periodic jobs. Adaptation means altering runtime options such as \texttt{message\_size}, \texttt{num\_counters}, and \texttt{num\_splitters}, which determines, e.g., how many messages are cached/processed simultaneously. The changing environments are related to the workload and type of a given micro-batch of jobs. 
%
%\textsc{Keras/DNN:} the deep neural network (DNN) from the well-known \textsc{Keras} framework for classification tasks as part of a learning system. When deployed and trained, the system classifies newly given samples. Adaptation refers to adjust options, e.g., \texttt{batch\_size} and \texttt{num\_filters}, for (re-)training the network in the system. The environment can change based on the given dataset for training.
%
%\textsc{x264:} A system for encoding videos. Adaptation means tuning runtime options includes \texttt{no\_mbtree}, \texttt{bframes}, and \texttt{ip\_ratio}, which are the keys for converting the video. The environment is determined by the sizes and frames of different videos.
%
%\textsc{Spear:} A strength bit-vector arithmetic decision procedure and a Boolean satisfiability (SAT) solver. Adaptation is achieved via changing the options on the logic of finding satisfiability, such as \texttt{sp\_phase\_dec\_heur} and \texttt{sp\_resolution}. The environment corresponds to the complexity/scale of the SAT problem to be solved.



%More detailed information about the SASs has been shown in Table~\ref{tb:sys}, 





%
%\subsection{Statistical Validation}
%
%To ensure the statistical significance of the results, we use: 
%
%\begin{itemize}
%  
%   
%  \item \textbf{Non-parametric test:} To verify statistical significance between two sets of values, we leverage the non-paired Wilcoxon rank-sum test~\cite{Wilcoxon1945IndividualCB} --- a widely applied non-parametric test in software engineering research and has been recommended for its strong statistical power on pairwise comparisons~\cite{ArcuriB11}. The standard $a=0.05$ is used as the significance level.
%   
%  %To ensure the resulted differences are not generated from a trivial effect,
%   
%   \item \textbf{Inter-correlations test:} Since the fitness landscape analysis involves a few correlations (e.g., FDC), we need to understand whether the difference between two correlations are statistically significant or not, and hence draw reasonable conclusions with respect to the planning landscapes under different environments. To that end, we adopt Fisher's transformation~\cite{fisher1915frequency} to find the z-score, which is then interpreted using Zou's confidence interval~\cite{zou2007toward} under a significance level of $0.05$. We leverage the \texttt{cocor} library\footnote{\textcolor{blue}{\texttt{\url{http://comparingcorrelations.org/}}}} in this work. 
%   
%   
%
%
%\end{itemize}
%
%For all cases, If the $p<0.05$, we say the magnitude of differences in the comparisons are significant. 

%\subsection{Methodology}

%talk about the method in the result




==> tables/rq1.tex <==


% CS Table for RQ2
\begin{table}[t!]
%\caption{Comparing \textsc{Flash} consolidated by our MOO$+$ model with the original \textsc{Flash} over 50 runs. The format is the same as Table~\ref{tb:rq1}.}
\caption{Statistical test on the FDC coefficient ($\varrho$) between all pairs of environments.}
%There exist N/A as \textsc{x264} and \textsc{Spear} do not have $E_4$.
    \label{tb:rq1}
   \footnotesize
    %\setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\columnwidth}
     

    \begin{tabular}{ccccc} \toprule
    \textbf{}&\textsc{Storm}&\textsc{Keras/DNN}&\textsc{x264}&\textsc{Spear}\\ \midrule
    
    $E_1 : E_2$&0.4742&\textbf{0.0215}&\textbf{$<$0.0001}&\textbf{0.0004} \\
    $E_1 : E_3$&\textbf{$<$0.0001}&\textbf{$<$0.0001}&\textbf{0.0151}&\textbf{$<$0.0001}\\
    $E_1 : E_4$&\textbf{0.0021}&\textbf{$<$0.0001}&N/A&N/A \\
    $E_2 : E_3$&\textbf{$<$0.0001}&\textbf{$<$0.0001}&0.0971&\textbf{$<$0.0001} \\
    $E_2 : E_4$&\textbf{0.0002}&\textbf{0.0001}&N/A&N/A \\
    $E_3 : E_4$&\textbf{$<$0.0001}&0.4454&N/A&N/A \\
    
    
    
    
    \bottomrule
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table}




==> tables/rq2.tex <==


% CS Table for RQ2
\begin{table}[t!]
%\caption{Comparing \textsc{Flash} consolidated by our MOO$+$ model with the original \textsc{Flash} over 50 runs. The format is the same as Table~\ref{tb:rq1}.}
\caption{Statistical test on the Correlation Length ($\ell$) between all pairs of environments for each SAS.}

%using Fisher's Transformation [] and Zou's confidence interval []. The statistically significant ones ($p<0.05$) are highlighted in bold
    \label{tb:rq2}
    \footnotesize
    %\setlength{\tabcolsep}{1mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\columnwidth}
     

    \begin{tabular}{ccccc} \toprule
    \textbf{}&\textsc{Storm}&\textsc{Keras/DNN}&\textsc{x264}&\textsc{Spear}\\ \midrule
    
    $E_1 : E_2$&0.7340&0.8712&0.8802&0.9142 \\
    $E_1 : E_3$&\textbf{0.029}&0.8095&0.6799&0.9757 \\
    $E_1 : E_4$&0.0516&0.8012&N/A&N/A \\
    $E_2 : E_3$&0.0659&0.9370&0.7934&0.8900 \\
    $E_2 : E_4$&0.1081&0.9285&N/A&N/A \\
    $E_3 : E_4$&0.8163&0.9914&N/A&N/A \\
    
    
    
    
    \bottomrule
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table}




==> tables/rq4-no-reversed-local-to-global.tex <==


% CS Table for RQ2
\begin{table*}[t!]
%In that regard, G$\rightarrow$L shows whether the global optimum in $E_x$ would become a local optimum in $E_y$ (Note that the global optimum adaptation plan(s) is often different for each environment); \cmark and \xmark~denote true and false, respectively. L$\rightarrow$L shows the \% of the local optima in $E_x$ that are also the local optima under $E_y$
\caption{The patterns on the global and local optima adaptation plans shared between different environments of the SASs studied. $A_1$, $A_2$, and $A_3$ refer to the three aspects assessed. $E_x$$\rightarrow$$E_y$ means the environment changes from $E_x$ to $E_y$. For $A_1$ and $A_2$, \cmark and \xmark~denote ``Yes'' and ``No'', respectively.}
    \label{tb:rq4}
   % \footnotesize
    %\setlength{\tabcolsep}{1.2mm}
  \begin{center}
    \begin{adjustbox}{max width = 1\textwidth}
     

    \begin{tabular}{cccc|ccc|ccc|ccc} \toprule
    \textbf{}& \multicolumn{3}{c|}{\textsc{Storm}}& \multicolumn{3}{c|}{\textsc{Keras/DNN}}& \multicolumn{3}{c|}{\textsc{x264}}& \multicolumn{3}{c}{\textsc{Spear}}\\ \cmidrule{2-13}
    
   \textbf{}&$A_1$&$A_2$&$A_3$&$A_1$&$A_2$&$A_3$&$A_1$&$A_2$&$A_3$&$A_1$&$A_2$&$A_3$\\ \midrule
    
 $E_1$$\rightarrow$$E_2$&\cmark&\xmark&56\%&\cmark&\cmark&31\%&\xmark&\cmark&85\%&\cmark&\xmark&18\% \\   
 
 $E_2$$\rightarrow$$E_1$&\cmark&\cmark&44\%&\cmark&\cmark&13\%&\xmark&\cmark&86\%&\cmark&\cmark&19\% \\   
  
 $E_1$$\rightarrow$$E_3$&\xmark&\cmark&38\%&\cmark&\xmark&95\%&\xmark&\cmark&85\%&\cmark&\xmark&47\% \\   
 
 $E_3$$\rightarrow$$E_1$&\xmark&\cmark&50\%&\cmark&\cmark&20\%&\xmark&\cmark&87\%&\cmark&\cmark&17\% \\ 
 
 $E_1$$\rightarrow$$E_4$&\xmark&\xmark&10\%&\cmark&\xmark&100\%&N/A&N/A&N/A&N/A&N/A&N/A \\ 
 
 $E_4$$\rightarrow$$E_1$&\xmark&\cmark&49\%&\cmark&\cmark&11\%&N/A&N/A&N/A&N/A&N/A&N/A  \\ 
 
 $E_2$$\rightarrow$$E_3$&\cmark&\cmark&38\%&\cmark&\xmark&63\%&\cmark&\xmark&86\%&\cmark&\xmark&65\% \\ 
 
 $E_3$$\rightarrow$$E_2$&\cmark&\xmark&64\%&\cmark&\cmark&33\%&\cmark&\xmark&88\%&\cmark&\cmark&23\% \\ 
 
 $E_2$$\rightarrow$$E_4$&\cmark&\cmark&11\%&\cmark&\xmark&100\%&N/A&N/A&N/A&N/A&N/A&N/A  \\ 
 
 $E_4$$\rightarrow$$E_2$&\cmark&\xmark&72\%&\cmark&\cmark&28\%&N/A&N/A&N/A&N/A&N/A&N/A  \\ 
 
 $E_3$$\rightarrow$$E_4$&\cmark&\cmark&25\%&\cmark&\xmark&100\%&N/A&N/A&N/A&N/A&N/A&N/A  \\ 
 
 $E_4$$\rightarrow$$E_3$&\cmark&\xmark&98\%&\cmark&\cmark&53\%&N/A&N/A&N/A&N/A&N/A&N/A  \\ 
  
    %19/36
    
    
    \bottomrule
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}




==> tables/rw.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	%\footnotesize
	
	\caption{Simple Random Walk Planner for SASs}
	\label{alg:rw}
	\KwIn{Adaptation plan space $\mathcal{V}$; step size $s$; walk length $p$}

	%\kwDeclare{$s_{best}$ the best adaptation plan on so far}
         \KwOut{the best adaptation plan found in the random walk}
	Randomly initialize a current plan $\vect{x}$ from $\mathcal{V}$\\

	\While{$i \leq p$}
	{  
	        $\vect{x'}$ = randomly choose a plan from the neighborhood of $\vect{x}$ with a radius of $s$.	\\
	          \If{$\vect{x'}$ has better performance than $\vect{x}$} {
	          $\vect{x} = \vect{x'}$ \\
	          }
		$i$++\\
	}
	
	\Return $\vect{x}$
	
\end{algorithm}
